FlightLLM: Efficient Large Language Model Inference with a Complete Mapping Flow on FPGAs

Transformer-based Large Language Models (LLMs) have made a significant impact on various domains. However, LLMs' efficiency suffers from both heavy computation and memory overheads. Compression techniques like sparsification and quantization are commonly used to mitigate the gap between LLM's computation/memory overheads and hardware capacity. However, existing GPU and transformer-based accelerators cannot efficiently process compressed LLMs, due to the following unresolved challenges: low computational efficiency, underutilized memory bandwidth, and large compilation overheads. This paper proposes FlightLLM, enabling efficient LLMs inference with a complete mapping flow on FPGAs. In FlightLLM, we highlight an innovative solution that the computation and memory overhead of LLMs can be solved by utilizing FPGA-specific resources (e.g., DSP48 and heterogeneous memory hierarchy). We propose a configurable sparse DSP chain to support different sparsity patterns with high computation efficiency. Second, we propose an always-on-chip decode scheme to boost memory bandwidth with mixed-precision support. Finally, to make FlightLLM available for real-world LLMs, we propose a length adaptive compilation method to reduce the compilation overhead. Implemented on the Xilinx Alveo U280 FPGA, FlightLLM achieves 6.0$\times$ higher energy efficiency and 1.8$\times$ better cost efficiency against commercial GPUs (e.g., NVIDIA V100S) on modern LLMs (e.g., LLaMA2-7B) using vLLM and SmoothQuant under the batch size of one. FlightLLM beats NVIDIA A100 GPU with 1.2$\times$ higher throughput using the latest Versal VHK158 FPGA.

==> content/overview.tex <==
%% ----------------------------------------------------------------
\section{Overview}

\subsection{Methodology Overview}
\todo{unify Figure and Fig.}

\todo{Mentions the importance of non-batched input.}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/Background/overview.png}
%   % \vspace{-15pt}
%   \caption{PLACEHOLDER: The overview}
%   % \vspace{-10pt}
%   \label{fig:overview}
% \end{figure}

\subsection{Mapping Flow Overview}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/Software/compile_flow.pdf}
  \vspace{-15pt}
  \caption{The overall deployment flow}
  \vspace{-10pt}
  \label{fig:compile_flow}
\end{figure}

Figure \ref{fig:compile_flow} shows our entire deployment flow. First, the original LLM model undergoes sparsification and quantization to create a compressed LLM model. Subsequently, the intermediate representation (IR) is exported, encompassing the model's structure, weights, sparse indexes, and attention masks, which is achieved through automated parsing of the model's structure. Following that, the generated IR undergoes optimization, which involves operations like removing the \texttt{view()} layers that do not impact the data arrangement and performing layer fusion. More specifically, the attention layer will be fused with the softmax layer, and the linear layer will be fused with ReLU, SiLU, and element-wise layers. Subsequently, all the data in the optimized IR will be assigned HBM or DDR storage addresses. Additionally, the data stored in the HBM will be partitioned into appropriate channels to prevent inefficient access across different channels, thus leveraging the FPGA's high bandwidth effectively. Lastly, the compiler will generate binary instructions for hardware operations using the optimized IR and schedule the on-chip buffer according to manually defined templates.

In addition, we also support generating corresponding RTL for different FPGA platforms. Specifically, the RTL Generator takes parameters of different FPGA platforms (including the amount of DSP, the capacity and bandwidth of HBM/DDR and on-chip RAM resources) to dynamically adjust the computing parallelism and buffer size of the proposed hardware architecture. This is done to generate corresponding RTL code for implementation and configurations for compilation, in order to maximize the optimal performance on different platforms.



==> content/related-work.tex <==
\subsection{Related Work}
% \todo{discuss more about the efficient LLMs}
\subsubsection{Efficient Transformer}

To tackle the extreme overhead of LLMs, various compression techniques are commonly used.
Quantization~\citep{dettmers2022llm_int8, frantar2022gptq, yao2022zeroquant, xiao2023smoothquant,lin2023awq} approaches use low-bit integers to substitute the 16-bit floating point parameters and activations for inference. 
Unlike small-sized models, LLMs often generate outlier activations with large magnitude, leading to large quantization error and accuracy loss for trivial quantization methods~\citep{dettmers2022llm_int8}. 
State-of-the-art solutions try to solve the outlier problem through weight-activation scale transformation~\citep{xiao2023smoothquant} and salient channel scaling~\citep{lin2023awq}, pushing the limit of weight bit width to 4 bits on GPUs.
However, given the lack of mix-precision support of GPU, no previous work utilizes mix-precision quantization to reduce the bit width further to the best of our knowledge.

Sparse attention~\citep{child2019spTrans, zaheer2020bigbird, beltagy2020longformer, wang2021spatten, chen2023dynamic_nm} and weight pruning~\citep{frantar2023sparsegpt, kwon2022fast} approaches skip part of the attention matrix or weight matrix computing according to the defined sparse pattern. Various sparse patterns are proposed for different tasks and transformers, including local diagonal pattern~\citep{beltagy2020longformer}, block sparse~\citep{child2019spTrans, zaheer2020bigbird, kitaev2020reformer, kwon2022fast}, N:M sparse pattern~\citep{chen2023dynamic_nm, frantar2023sparsegpt}, row-column skipping pattern~\citep{wang2021spatten}, unstructured pattern~\citep{frantar2023sparsegpt} and so on.
Previous work pushes the limit of attention and weight sparsity to 67\% (2 thousand tokens by~\citep{zaheer2020bigbird}) and 60\% (OPT-175B model by \citep{frantar2023sparsegpt}) or even higher. However, most of them fail to demonstrate corresponding speedup on GPU due to the lack of sparse computation support of the hardware~\citep{tay2020LRA}.

\subsubsection{LLM-related Accelerators}
Targeted at transformer models, previous work~\cite{li2020ftrans,ham2020a3,isca2021elsa,micro2021sanger,wang2021spatten,micro2022DFX,micro2022bufferfly,hpca23flat,isca2023fact,wang2023cosa} propose customized architecture design for transformer models. Some work~\cite{micro2021sanger,wang2023cosa} focuses on optimizing on-chip dataflow. They use techniques like operator fusion~\citep{micro2021sanger} and co-operative systolic arrays~\citep{wang2023cosa} to improve on-chip data reuse and reduce memory access. 
Some work~\cite{CTA2023, micro2021sanger,wang2021spatten,micro2022bufferfly,li2020ftrans,isca2021elsa} lay more emphasis on accelerating sparse attention.
They design specialized architectures to fully utilize the pre-defined static attention pattern~\cite{micro2022bufferfly,li2020ftrans} or dynamically generated attention pattern~\cite{isca2023fact,CTA2023,wang2021spatten,micro2021sanger}.
Recently, FACT~\cite{isca2023fact} points out the importance of compressing linear layers with mixed-precision quantization to help reduce latency.
However, these methods cannot accelerate the decode stage of LLMs since they mainly focus on the \textit{prefill} stage for discriminative models, like medium-sized BERT~\cite{devlin2019bert} model.
% SpAtten~\cite{wang2021spatten} reduces attention computation in both \textit{prefill} and \textit{decode} stage by directly pruning attention heads. 

Recent work DFX~\cite{micro2022DFX} emphasizes the acceleration of the decode stage of LLMs.
It builds a multi-FPGA cluster with model parallelism for GPT-2. It mainly optimizes tiling scheme and dataflow to fully utilize all the channels of HBMs. However, it lacks hardware support for model compression of LLMs, making it hard to further expand model size or maximum token size.

